Exploiting the Matching Information in the Support Set for Few Shot Event Classification

The existing event classification (EC) work primarily focuseson the traditional supervised learning setting in which models are unableto extract event mentions of new/unseen event types. Few-shot learninghas not been investigated in this area although it enables EC models toextend their operation to unobserved event types. To fill in this gap, inthis work, we investigate event classification under the few-shot learningsetting. We propose a novel training method for this problem that exten-sively exploit the support set during the training process of a few-shotlearning model. In particular, in addition to matching the query exam-ple with those in the support set for training, we seek to further matchthe examples within the support set themselves. This method providesmore training signals for the models and can be applied to every metric-learning-based few-shot learning methods. Our extensive experiments ontwo benchmark EC datasets show that the proposed method can improvethe best reported few-shot learning models by up to 10% on accuracyfor event classification

==> tbl-dataset.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{|l|l|c|c|}
    \hline
         & & ACE-2005 & TAC-KBP\\
        \hline 
        \multirow{3}{*}{\#Samples} & Train & 2,844 & 7,503\\
        %& Dev & 1.114 & 2.241\\
        %& Test &1.122 & 2.250\\
        & Test &1,118 & 2,245\\
        & Dev & 1,118 & 2,245\\
        \hline
        \multirow{3}{*}{\#Subtypes}& Train & 21 & 24\\
        & Dev & 11 & 14 \\
        & Test & 11 & 14 \\
        \hline
    \end{tabular}
    \caption{Dataset statistics.}
    \label{tbl:statistics}
\end{table}

==> tbl-ed-ace.tex <==

In addition to event classification FSL, we also proposed to turn supervised-learning event detection into FSL event detection (ED). In order to do so, we formalize ED under N-way K-shot N-other FSL setting. Instead of using N-clusters, representing classes, of samples in the support set, we add N clusters of the same \textit{null} class, hence, we call this \textbf{N-other}. We sample these clusters randomly from a pool of non-event samples in the way that all null clusters are disjoint. During testing, whenever model predict a label to be one of the N-other clusters, we consider it as a single "Null" labels. We train the following model using the same hyperparameters as presented above.
Following previous studies, we evaluate all the models using micro F1-score. The results of four models (i.e. Matching, Proto, Proto + Att, Relation) using Transformer encoder under 5-way 5-shot 5-other and 10-way 10-shot 10-other are presented in table \ref{tbl:ed-ace}. 

As can be seen from the table, comparing models without LoLoss, Proto+Att delivers the highest F-score on 5-way 5-shot 5-other setting while Proto achieves the highest performance on 10-way 10-shot 10-other setting at 71.14\%. Importantly, adding LoLoss to the training procedure improve the performance of 0.8\% to 4.5\% on every models. This experiment, again, confirm the effectiveness of exploiting matching information between samples in the support set.

\begin{table}[]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Model} &  \textbf{5-way 5-shot 5-other} & \textbf{10-way 10-shot 10-other} \\
\hline
Matching         & 73.27 & 65.68 \\  
Matching+LoLoss  & \textbf{74.48} & \textbf{70.19} \\ \hline
Proto            & 74.27 & 71.14 \\  
Proto+LoLoss     & \textbf{75.72} & \textbf{71.80} \\ \hline
Proto+Att        & 74.76 & 70.04 \\  
Proto+Att+LoLoss & \textbf{75.94} & \textbf{71.87} \\ \hline
Relation         & 38.68 & 29.43 \\  
Relation+LoLoss  & \textbf{39.44} & \textbf{30.24} \\ \hline
\end{tabular}
\caption{Event detection performance on ACE-2005 dataset. \textbf{+LoLoss} indicates the model with auxiliary loss.}
\label{tbl:ed-ace}
\end{table}
